Track Reconstruction Performance in CMS

The expected performance of track reconstruction with LHC events using the CMS silicon tracker is presented. Track finding and fitting is accomplished with Kalman Filter techniques that achieve efficiencies above 99% on single muons with pT>1 GeV/c. Difficulties arise in the context of standard LHC events with a high density of charged particles, where the rate of fake combinatorial tracks is very large for low pT tracks, and nuclear interactions in the tracker material reduce the tracking efficiency for charged hadrons. Recent improvements with the CMS track reconstruction now allow to efficiently reconstruct charged tracks with pT down to few hundred MeV/c and as few as three crossed layers, with a very small fake fraction, by making use of an optimal rejection of fake tracks in conjunction with an iterative tracking procedure.

==> pdefs.tex <==
\newcommand{\fastkt}{Fast $k_\mathrm{T}$\xspace}
\newcommand{\siscone}{SISCone\xspace}
\newcommand{\midpoint}{Midpoint Cone\xspace}
\newcommand{\itcone}{Iterative Cone\xspace}

\newcommand{\cmsswfive}{CMSSW\_1\_5\_2\xspace}
\newcommand{\cmsswsix}{CMSSW\_1\_6\_X\xspace}

\newcommand{\DeltaR}{\ensuremath{\Delta R}\xspace}
\newcommand{\kt}{\ensuremath{k_{\mathrm{T}}}\xspace}
\newcommand{\pt}{\ensuremath{p_{\mathrm{T}}}\xspace}
\newcommand{\ptgen}{\ensuremath{p_{\mathrm{T}}^{\mathrm{gen}}}\xspace}
\newcommand{\ptcorr}{\ensuremath{p_{\mathrm{T}}^{\mathrm{corr}}}\xspace}
\newcommand{\et}{\ensuremath{E_{\mathrm{T}}}\xspace}
\newcommand{\etgen}{\ensuremath{E_{\mathrm{T}}^{\mathrm{gen}}}\xspace}
\newcommand{\etcorr}{\ensuremath{E_{\mathrm{T}}^{\mathrm{corr}}}\xspace}
\newcommand{\etagen}{\ensuremath{\eta^{\mathrm{gen}}}\xspace}
\newcommand{\phigen}{\ensuremath{\phi^{\mathrm{gen}}}\xspace}
\newcommand{\MeV}{\,\ensuremath{\mathrm{Me\kern-0.1em V}}\xspace}
\newcommand{\GeV}{\,\ensuremath{\mathrm{Ge\kern-0.1em V}}\xspace}

\newcommand{\ipb}{\,pb^{-1}\xspace}
\newcommand{\ifb}{\,fb^{-1}\xspace}

\newcommand{\ttbar}{\ensuremath{t\bar{t}}\xspace}
\newcommand{\mtop}{\ensuremath{m_{t}}\xspace}
\newcommand{\mW}{\ensuremath{m_{W}}\xspace}

\newcommand{\alpgen}{{\sc Alpgen}\xspace}

